Imprints of a Supercooled Phase Transition in the Gravitational Wave Spectrum from a Cosmic String network

A network of cosmic strings (CS), if present, would continue emitting gravitational waves (GW) as it evolves throughout the history of the Universe. This results in a characteristic broad spectrum making it a perfect source to infer the expansion history. In particular, a short inflationary period caused by a supercooled phase transition would cause a drop in the spectrum at frequencies corresponding to that event. However, the impact on the spectrum is similar to the ones caused by an early matter-dominated era or from particle production, making it difficult to disentangle these different physical origins. We point out that, in the case of a short inflationary period, the GW spectrum receives an additional contribution from the phase transition itself. This leads to a characteristic imprint of a peak on top of a wide plateau both visible at future GW observatories.

==> main_bib <==
@article{Caprini:2018mtu,
    author = "Caprini, Chiara and Figueroa, Daniel G.",
    title = "{Cosmological Backgrounds of Gravitational Waves}",
    eprint = "1801.04268",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1361-6382/aac608",
    journal = "Class. Quant. Grav.",
    volume = "35",
    number = "16",
    pages = "163001",
    year = "2018"
}


@article{Giovannini:1998bp,
    author = "Giovannini, Massimo",
    title = "{Gravitational waves constraints on postinflationary phases stiffer than radiation}",
    eprint = "hep-ph/9806329",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.58.083504",
    journal = "Phys. Rev. D",
    volume = "58",
    pages = "083504",
    year = "1998"
}


@article{Giovannini:2009kg,
    author = "Giovannini, Massimo",
    title = "{Stochastic backgrounds of relic gravitons: a theoretical appraisal}",
    eprint = "0901.3026",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "CERN-PH-TH-2008-252",
    doi = "10.1186/1754-0410-4-1",
    journal = "PMC Phys. A",
    volume = "4",
    pages = "1",
    year = "2010"
}


@article{Riazuelo:2000fc,
    author = "Riazuelo, Alain and Uzan, Jean-Philippe",
    title = "{Quintessence and gravitational waves}",
    eprint = "astro-ph/0004156",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.62.083506",
    journal = "Phys. Rev. D",
    volume = "62",
    pages = "083506",
    year = "2000"
}


@article{Sahni:2001qp,
    author = "Sahni, Varun and Sami, M. and Souradeep, Tarun",
    title = "{Relic gravity waves from brane world inflation}",
    eprint = "gr-qc/0105121",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.65.023518",
    journal = "Phys. Rev. D",
    volume = "65",
    pages = "023518",
    year = "2002"
}


@article{Seto:2003kc,
    author = "Seto, Naoki and Yokoyama, Jun'Ichi",
    title = "{Probing the equation of state of the early universe with a space laser interferometer}",
    eprint = "gr-qc/0305096",
    archivePrefix = "arXiv",
    reportNumber = "OU-TAP-206",
    doi = "10.1143/JPSJ.72.3082",
    journal = "J. Phys. Soc. Jap.",
    volume = "72",
    pages = "3082--3086",
    year = "2003"
}


@article{Tashiro:2003qp,
    author = "Tashiro, Hiroyuki and Chiba, Takeshi and Sasaki, Misao",
    title = "{Reheating after quintessential inflation and gravitational waves}",
    eprint = "gr-qc/0307068",
    archivePrefix = "arXiv",
    doi = "10.1088/0264-9381/21/7/004",
    journal = "Class. Quant. Grav.",
    volume = "21",
    pages = "1761--1772",
    year = "2004"
}


@article{Nakayama:2008ip,
    author = "Nakayama, Kazunori and Saito, Shun and Suwa, Yudai and Yokoyama, Jun'ichi",
    title = "{Space laser interferometers can determine the thermal history of the early Universe}",
    eprint = "0802.2452",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "RESCEU-2-08, UTAP-594",
    doi = "10.1103/PhysRevD.77.124001",
    journal = "Phys. Rev. D",
    volume = "77",
    pages = "124001",
    year = "2008"
}


@article{Nakayama:2008wy,
    author = "Nakayama, Kazunori and Saito, Shun and Suwa, Yudai and Yokoyama, Jun'ichi",
    title = "{Probing reheating temperature of the universe with gravitational wave background}",
    eprint = "0804.1827",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph",
    reportNumber = "RESCEU-7-08, UTAP-596",
    doi = "10.1088/1475-7516/2008/06/020",
    journal = "JCAP",
    volume = "06",
    pages = "020",
    year = "2008"
}


@article{Durrer:2011bi,
    author = "Durrer, Ruth and Hasenkamp, Jasper",
    title = "{Testing Superstring Theories with Gravitational Waves}",
    eprint = "1105.5283",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    doi = "10.1103/PhysRevD.84.064027",
    journal = "Phys. Rev. D",
    volume = "84",
    pages = "064027",
    year = "2011"
}


@article{Kuroyanagi:2011fy,
    author = "Kuroyanagi, Sachiko and Nakayama, Kazunori and Saito, Shun",
    title = "{Prospects for determination of thermal history after inflation with future gravitational wave detectors}",
    eprint = "1110.4169",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "ICRR-REPORT-597-2011-14, UT-11-35",
    doi = "10.1103/PhysRevD.84.123513",
    journal = "Phys. Rev. D",
    volume = "84",
    pages = "123513",
    year = "2011"
}


@article{Kuroyanagi:2018csn,
    author = "Kuroyanagi, Sachiko and Chiba, Takeshi and Takahashi, Tomo",
    title = "{Probing the Universe through the Stochastic Gravitational Wave Background}",
    eprint = "1807.00786",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1475-7516/2018/11/038",
    journal = "JCAP",
    volume = "11",
    pages = "038",
    year = "2018"
}


@article{Jinno:2012xb,
    author = "Jinno, Ryusuke and Moroi, Takeo and Nakayama, Kazunori",
    title = "{Probing dark radiation with inflationary gravitational waves}",
    eprint = "1208.0184",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "UT-12-26",
    doi = "10.1103/PhysRevD.86.123502",
    journal = "Phys. Rev. D",
    volume = "86",
    pages = "123502",
    year = "2012"
}


@article{Lasky:2015lej,
    author = "Lasky, Paul D. and others",
    title = "{Gravitational-wave cosmology across 29 decades in frequency}",
    eprint = "1511.05994",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevX.6.011035",
    journal = "Phys. Rev. X",
    volume = "6",
    number = "1",
    pages = "011035",
    year = "2016"
}


@article{Li:2016mmc,
    author = "Li, Bohua and Shapiro, Paul R. and Rindler-Daller, Tanja",
    title = "{Bose-Einstein-condensed scalar field dark matter and the gravitational wave background from inflation: new cosmological constraints and its detectability by LIGO}",
    eprint = "1611.07961",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.96.063505",
    journal = "Phys. Rev. D",
    volume = "96",
    number = "6",
    pages = "063505",
    year = "2017"
}


@article{Saikawa:2018rcs,
    author = "Saikawa, Ken'ichi and Shirai, Satoshi",
    title = "{Primordial gravitational waves, precisely: The role of thermodynamics in the Standard Model}",
    eprint = "1803.01038",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IPMU18-0037, MPP-2018-19",
    doi = "10.1088/1475-7516/2018/05/035",
    journal = "JCAP",
    volume = "05",
    pages = "035",
    year = "2018"
}


@article{Caldwell:2018giq,
    author = "Caldwell, Robert R. and Smith, Tristan L. and Walker, Devin G. E.",
    title = "{Using a Primordial Gravitational Wave Background to Illuminate New Physics}",
    eprint = "1812.07577",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.100.043513",
    journal = "Phys. Rev. D",
    volume = "100",
    number = "4",
    pages = "043513",
    year = "2019"
}


@article{Bernal:2019lpc,
    author = "Bernal, Nicol\'as and Hajkarim, Fazlollah",
    title = "{Primordial Gravitational Waves in Nonstandard Cosmologies}",
    eprint = "1905.10410",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.100.063502",
    journal = "Phys. Rev. D",
    volume = "100",
    number = "6",
    pages = "063502",
    year = "2019"
}


@article{Figueroa:2019paj,
    author = "Figueroa, Daniel G. and Tanin, Erwin H.",
    title = "{Ability of LIGO and LISA to probe the equation of state of the early Universe}",
    eprint = "1905.11960",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1475-7516/2019/08/011",
    journal = "JCAP",
    volume = "08",
    pages = "011",
    year = "2019"
}


@article{DEramo:2019tit,
    author = "D'Eramo, Francesco and Schmitz, Kai",
    title = "{Imprint of a scalar era on the primordial spectrum of gravitational waves}",
    eprint = "1904.07870",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevResearch.1.013010",
    journal = "Phys. Rev. Research.",
    volume = "1",
    pages = "013010",
    year = "2019"
}


@article{Cui:2017ufi,
    author = "Cui, Yanou and Lewicki, Marek and Morrissey, David E. and Wells, James D.",
    title = "{Cosmic Archaeology with Gravitational Waves from Cosmic Strings}",
    eprint = "1711.03104",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "KCL-PH-TH-2017-51",
    doi = "10.1103/PhysRevD.97.123505",
    journal = "Phys. Rev. D",
    volume = "97",
    number = "12",
    pages = "123505",
    year = "2018"
}


@article{Cui:2018rwi,
    author = "Cui, Yanou and Lewicki, Marek and Morrissey, David E. and Wells, James D.",
    title = "{Probing the pre-BBN universe with gravitational waves from cosmic strings}",
    eprint = "1808.08968",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "KCL-PH-TH/2018-47",
    doi = "10.1007/JHEP01(2019)081",
    journal = "JHEP",
    volume = "01",
    pages = "081",
    year = "2019"
}


@article{Auclair:2019wcv,
    author = "Auclair, Pierre and others",
    title = "{Probing the gravitational wave background from cosmic strings with LISA}",
    eprint = "1909.00819",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1475-7516/2020/04/034",
    journal = "JCAP",
    volume = "04",
    pages = "034",
    year = "2020"
}


@article{Guedes:2018afo,
    author = "Guedes, G. S. F. and Avelino, P. P. and Sousa, L.",
    title = "{Signature of inflation in the stochastic gravitational wave background generated by cosmic string networks}",
    eprint = "1809.10802",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.98.123505",
    journal = "Phys. Rev. D",
    volume = "98",
    number = "12",
    pages = "123505",
    year = "2018"
}


@article{Ramberg:2019dgi,
    author = "Ramberg, Nicklas and Visinelli, Luca",
    title = "{Probing the Early Universe with Axion Physics and Gravitational Waves}",
    eprint = "1904.05707",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.99.123513",
    journal = "Phys. Rev. D",
    volume = "99",
    number = "12",
    pages = "123513",
    year = "2019"
}


@article{Chang:2019mza,
    author = "Chang, Chia-Feng and Cui, Yanou",
    title = "{Stochastic Gravitational Wave Background from Global Cosmic Strings}",
    eprint = "1910.04781",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1016/j.dark.2020.100604",
    journal = "Phys. Dark Univ.",
    volume = "29",
    pages = "100604",
    year = "2020"
}


@article{Vilenkin:1981bx,
    author = "Vilenkin, A.",
    title = "{Gravitational radiation from cosmic strings}",
    doi = "10.1016/0370-2693(81)91144-8",
    journal = "Phys. Lett. B",
    volume = "107",
    pages = "47--50",
    year = "1981"
}


@article{Hogan:1984is,
    author = "Hogan, C. J. and Rees, M. J.",
    editor = "Lindley, D. and Kolb, Edward W. and Schramm, D. N.",
    title = "{Gravitational interactions of cosmic strings}",
    doi = "10.1038/311109a0",
    journal = "Nature",
    volume = "311",
    pages = "109--113",
    year = "1984"
}


@article{Vachaspati:1984gt,
    author = "Vachaspati, Tanmay and Vilenkin, Alexander",
    title = "{Gravitational Radiation from Cosmic Strings}",
    reportNumber = "HUTP-84/A065",
    doi = "10.1103/PhysRevD.31.3052",
    journal = "Phys. Rev. D",
    volume = "31",
    pages = "3052",
    year = "1985"
}


@article{Accetta:1988bg,
    author = "Accetta, Frank S. and Krauss, Lawrence M.",
    title = "{The stochastic gravitational wave spectrum resulting from cosmic string evolution}",
    reportNumber = "YCTP-P5-88",
    doi = "10.1016/0550-3213(89)90628-7",
    journal = "Nucl. Phys. B",
    volume = "319",
    pages = "747--764",
    year = "1989"
}


@article{Bennett:1990ry,
    author = "Bennett, David P. and Bouchet, Francois R.",
    title = "{Constraints on the gravity wave background generated by cosmic strings}",
    reportNumber = "UCRL-JC-105282",
    doi = "10.1103/PhysRevD.43.2733",
    journal = "Phys. Rev. D",
    volume = "43",
    pages = "2733--2735",
    year = "1991"
}


@article{Caldwell:1991jj,
    author = "Caldwell, R. R. and Allen, Bruce",
    title = "{Cosmological constraints on cosmic string gravitational radiation}",
    reportNumber = "WISC-MILW-91-TH-14",
    doi = "10.1103/PhysRevD.45.3447",
    journal = "Phys. Rev. D",
    volume = "45",
    pages = "3447--3468",
    year = "1992"
}


@article{Allen:1991bk,
    author = "Allen, Bruce and Shellard, E. P. S.",
    title = "{Gravitational radiation from cosmic strings}",
    reportNumber = "WISC-MILW-91-TH-12",
    doi = "10.1103/PhysRevD.45.1898",
    journal = "Phys. Rev. D",
    volume = "45",
    pages = "1898--1912",
    year = "1992"
}


@inproceedings{Battye:1997ji,
    author = "Battye, R. A. and Caldwell, R. R. and Shellard, E. P. S.",
    title = "{Gravitational waves from cosmic strings}",
    booktitle = "{Conference on Topological Defects and CMB}",
    eprint = "astro-ph/9706013",
    archivePrefix = "arXiv",
    reportNumber = "IMPERIAL-TP-95-96-30",
    pages = "11--31",
    month = "6",
    year = "1997"
}


@article{DePies:2007bm,
    author = "DePies, Matthew R. and Hogan, Craig J.",
    title = "{Stochastic Gravitational Wave Background from Light Cosmic Strings}",
    eprint = "astro-ph/0702335",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.75.125006",
    journal = "Phys. Rev. D",
    volume = "75",
    pages = "125006",
    year = "2007"
}


@article{Siemens:2006yp,
    author = "Siemens, Xavier and Mandic, Vuk and Creighton, Jolien",
    title = "{Gravitational wave stochastic background from cosmic (super)strings}",
    eprint = "astro-ph/0610920",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevLett.98.111101",
    journal = "Phys. Rev. Lett.",
    volume = "98",
    pages = "111101",
    year = "2007"
}


@article{Olmez:2010bi,
    author = "Olmez, S. and Mandic, V. and Siemens, X.",
    title = "{Gravitational-Wave Stochastic Background from Kinks and Cusps on Cosmic Strings}",
    eprint = "1004.0890",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.81.104028",
    journal = "Phys. Rev. D",
    volume = "81",
    pages = "104028",
    year = "2010"
}


@article{Regimbau:2011bm,
    author = "Regimbau, Tania and Giampanis, Stefanos and Siemens, Xavier and Mandic, Vuk",
    title = "{The stochastic background from cosmic (super)strings: popcorn and (Gaussian) continuous regimes}",
    eprint = "1111.6638",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.85.066001",
    journal = "Phys. Rev. D",
    volume = "85",
    pages = "066001",
    year = "2012"
}


@article{Sanidas:2012ee,
    author = "Sanidas, S. A. and Battye, R. A. and Stappers, B. W.",
    title = "{Constraints on cosmic string tension imposed by the limit on the stochastic gravitational wave background from the European Pulsar Timing Array}",
    eprint = "1201.2419",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.85.122003",
    journal = "Phys. Rev. D",
    volume = "85",
    pages = "122003",
    year = "2012"
}


@article{Sanidas:2012tf,
    author = "Sanidas, Sotirios A. and Battye, Richard A. and Stappers, Benjamin W.",
    title = "{Projected constraints on the cosmic (super)string tension with future gravitational wave detection experiments}",
    eprint = "1211.5042",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/0004-637X/764/1/108",
    journal = "Astrophys. J.",
    volume = "764",
    pages = "108",
    year = "2013"
}


@article{Binetruy:2012ze,
    author = "Binetruy, Pierre and Bohe, Alejandro and Caprini, Chiara and Dufaux, Jean-Francois",
    title = "{Cosmological Backgrounds of Gravitational Waves and eLISA/NGO: Phase Transitions, Cosmic Strings and Other Sources}",
    eprint = "1201.0983",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    doi = "10.1088/1475-7516/2012/06/027",
    journal = "JCAP",
    volume = "06",
    pages = "027",
    year = "2012"
}


@article{Kuroyanagi:2012wm,
    author = "Kuroyanagi, Sachiko and Miyamoto, Koichi and Sekiguchi, Toyokazu and Takahashi, Keitaro and Silk, Joseph",
    title = "{Forecast constraints on cosmic string parameters from gravitational wave direct detection experiments}",
    eprint = "1202.3032",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.86.023503",
    journal = "Phys. Rev. D",
    volume = "86",
    pages = "023503",
    year = "2012"
}


@article{Kuroyanagi:2012jf,
    author = "Kuroyanagi, Sachiko and Miyamoto, Koichi and Sekiguchi, Toyokazu and Takahashi, Keitaro and Silk, Joseph",
    title = "{Forecast constraints on cosmic strings from future CMB, pulsar timing and gravitational wave direct detection experiments}",
    eprint = "1210.2829",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.87.023522",
    journal = "Phys. Rev. D",
    volume = "87",
    number = "2",
    pages = "023522",
    year = "2013",
    note = "[Erratum: Phys.Rev.D 87, 069903 (2013)]"
}


@article{Sousa:2016ggw,
    author = "Sousa, L. and Avelino, P. P.",
    title = "{Probing Cosmic Superstrings with Gravitational Waves}",
    eprint = "1606.05585",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.94.063529",
    journal = "Phys. Rev. D",
    volume = "94",
    number = "6",
    pages = "063529",
    year = "2016"
}


@article{Sousa:2020sxs,
    author = "Sousa, Lara and Avelino, Pedro P. and Guedes, Guilherme S. F.",
    title = "{Full analytical approximation to the stochastic gravitational wave background generated by cosmic string networks}",
    eprint = "2002.01079",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.101.103508",
    journal = "Phys. Rev. D",
    volume = "101",
    number = "10",
    pages = "103508",
    year = "2020"
}


@article{Creminelli:2001th,
    author = "Creminelli, Paolo and Nicolis, Alberto and Rattazzi, Riccardo",
    title = "{Holography and the electroweak phase transition}",
    eprint = "hep-th/0107141",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-2001-189",
    doi = "10.1088/1126-6708/2002/03/051",
    journal = "JHEP",
    volume = "03",
    pages = "051",
    year = "2002"
}


@article{Randall:2006py,
    author = "Randall, Lisa and Servant, Geraldine",
    title = "{Gravitational waves from warped spacetime}",
    eprint = "hep-ph/0607158",
    archivePrefix = "arXiv",
    reportNumber = "CERN-PH-TH-2006-133",
    doi = "10.1088/1126-6708/2007/05/054",
    journal = "JHEP",
    volume = "05",
    pages = "054",
    year = "2007"
}


@article{Nardini:2007me,
    author = "Nardini, Germano and Quiros, Mariano and Wulzer, Andrea",
    title = "{A Confining Strong First-Order Electroweak Phase Transition}",
    eprint = "0706.3388",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UAB-FT-632",
    doi = "10.1088/1126-6708/2007/09/077",
    journal = "JHEP",
    volume = "09",
    pages = "077",
    year = "2007"
}


@article{Konstandin:2011dr,
    author = "Konstandin, Thomas and Servant, Geraldine",
    title = "{Cosmological Consequences of Nearly Conformal Dynamics at the TeV scale}",
    eprint = "1104.4791",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2011/12/009",
    journal = "JCAP",
    volume = "12",
    pages = "009",
    year = "2011"
}


@article{vonHarling:2017yew,
    author = "von Harling, Benedict and Servant, Geraldine",
    title = "{QCD-induced Electroweak Phase Transition}",
    eprint = "1711.11554",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-17-056",
    doi = "10.1007/JHEP01(2018)159",
    journal = "JHEP",
    volume = "01",
    pages = "159",
    year = "2018"
}


@article{Iso:2017uuu,
    author = "Iso, Satoshi and Serpico, Pasquale D. and Shimada, Kengo",
    title = "{QCD-Electroweak First-Order Phase Transition in a Supercooled Universe}",
    eprint = "1704.04955",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "KEK-TH-1969, LAPTH-008-17",
    doi = "10.1103/PhysRevLett.119.141301",
    journal = "Phys. Rev. Lett.",
    volume = "119",
    number = "14",
    pages = "141301",
    year = "2017"
}


@article{Bruggisser:2018mrt,
    author = "Bruggisser, Sebastian and Von Harling, Benedict and Matsedonskyi, Oleksii and Servant, G\'eraldine",
    title = "{Electroweak Phase Transition and Baryogenesis in Composite Higgs Models}",
    eprint = "1804.07314",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-17-229",
    doi = "10.1007/JHEP12(2018)099",
    journal = "JHEP",
    volume = "12",
    pages = "099",
    year = "2018"
}


@article{Baratella:2018pxi,
    author = "Baratella, Pietro and Pomarol, Alex and Rompineve, Fabrizio",
    title = "{The Supercooled Universe}",
    eprint = "1812.06996",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP03(2019)100",
    journal = "JHEP",
    volume = "03",
    pages = "100",
    year = "2019"
}


@article{Agashe:2019lhy,
    author = "Agashe, Kaustubh and Du, Peizhi and Ekhterachian, Majid and Kumar, Soubhik and Sundrum, Raman",
    title = "{Cosmological Phase Transition of Spontaneous Confinement}",
    eprint = "1910.06238",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UMD-PP-019-05, YITP-SB-19-32",
    doi = "10.1007/JHEP05(2020)086",
    journal = "JHEP",
    volume = "05",
    pages = "086",
    year = "2020"
}


@article{DelleRose:2019pgi,
    author = "Delle Rose, Luigi and Panico, Giuliano and Redi, Michele and Tesi, Andrea",
    title = "{Gravitational Waves from Supercool Axions}",
    eprint = "1912.06139",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP04(2020)025",
    journal = "JHEP",
    volume = "04",
    pages = "025",
    year = "2020"
}


@article{vonHarling:2019gme,
    author = "Von Harling, Benedict and Pomarol, Alex and Pujol\`as, Oriol and Rompineve, Fabrizio",
    title = "{Peccei-Quinn Phase Transition at LIGO}",
    eprint = "1912.07587",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP04(2020)195",
    journal = "JHEP",
    volume = "04",
    pages = "195",
    year = "2020"
}


@article{Spokoiny:1993kt,
    author = "Spokoiny, Boris",
    title = "{Deflationary universe scenario}",
    eprint = "gr-qc/9306008",
    archivePrefix = "arXiv",
    reportNumber = "KUNS-1201",
    doi = "10.1016/0370-2693(93)90155-B",
    journal = "Phys. Lett. B",
    volume = "315",
    pages = "40--45",
    year = "1993"
}


@article{Joyce:1996cp,
    author = "Joyce, Michael",
    title = "{Electroweak Baryogenesis and the Expansion Rate of the Universe}",
    eprint = "hep-ph/9606223",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-96-098, CERN-TH-96-98",
    doi = "10.1103/PhysRevD.55.1875",
    journal = "Phys. Rev. D",
    volume = "55",
    pages = "1875--1878",
    year = "1997"
}


@article{Ellis:2018mja,
    author = "Ellis, John and Lewicki, Marek and No, Jos\'e Miguel",
    title = "{On the Maximal Strength of a First-Order Electroweak Phase Transition and its Gravitational Wave Signal}",
    eprint = "1809.08242",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "KCL-PH-TH/2018-46, CERN-TH/2018-197, IFT-UAM/CSIC-18-94, CERN-TH-2018-197",
    doi = "10.1088/1475-7516/2019/04/003",
    journal = "JCAP",
    volume = "04",
    pages = "003",
    year = "2019"
}


@article{Ellis:2019oqb,
    author = "Ellis, John and Lewicki, Marek and No, Jos\'e Miguel and Vaskonen, Ville",
    title = "{Gravitational wave energy budget in strongly supercooled phase transitions}",
    eprint = "1903.09642",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "KCL-PH-TH/2019-32, CERN-TH-2019-032, IFT-UAM/CSIC-19-32",
    doi = "10.1088/1475-7516/2019/06/024",
    journal = "JCAP",
    volume = "06",
    pages = "024",
    year = "2019"
}


@article{Ellis:2020nnr,
    author = "Ellis, John and Lewicki, Marek and Vaskonen, Ville",
    title = "{Updated predictions for gravitational waves produced in a strongly supercooled phase transition}",
    eprint = "2007.15586",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "KCL-PH-TH/2020-40, CERN-TH-2020-129",
    doi = "10.1088/1475-7516/2020/11/020",
    journal = "JCAP",
    volume = "11",
    pages = "020",
    year = "2020"
}


@article{Ellis:2020awk,
    author = "Ellis, John and Lewicki, Marek and No, Jos\'e Miguel",
    title = "{Gravitational waves from first-order cosmological phase transitions: lifetime of the sound wave source}",
    eprint = "2003.07360",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "KCL-PH-TH/2020-04, CERN-TH-2020-016, IFT-UAM/CSIC-20-35",
    doi = "10.1088/1475-7516/2020/07/050",
    journal = "JCAP",
    volume = "07",
    pages = "050",
    year = "2020"
}


@article{Guth:1979bh,
    author = "Guth, Alan H. and Tye, S. H. H.",
    title = "{Phase Transitions and Magnetic Monopole Production in the Very Early Universe}",
    reportNumber = "SLAC-PUB-2448, CLNS-79-441",
    doi = "10.1103/PhysRevLett.44.631",
    journal = "Phys. Rev. Lett.",
    volume = "44",
    pages = "631",
    year = "1980",
    note = "[Erratum: Phys.Rev.Lett. 44, 963 (1980)]"
}


@article{Guth:1981uk,
    author = "Guth, Alan H. and Weinberg, Erick J.",
    title = "{Cosmological Consequences of a First Order Phase Transition in the SU(5) Grand Unified Model}",
    reportNumber = "CU-TP-183",
    doi = "10.1103/PhysRevD.23.876",
    journal = "Phys. Rev. D",
    volume = "23",
    pages = "876",
    year = "1981"
}


@article{Kamionkowski:1993fg,
    author = "Kamionkowski, Marc and Kosowsky, Arthur and Turner, Michael S.",
    title = "{Gravitational radiation from first order phase transitions}",
    eprint = "astro-ph/9310044",
    archivePrefix = "arXiv",
    reportNumber = "IASSNS-HEP-93-44, FERMILAB-PUB-93-235-A",
    doi = "10.1103/PhysRevD.49.2837",
    journal = "Phys. Rev. D",
    volume = "49",
    pages = "2837--2851",
    year = "1994"
}


@article{Caprini:2019egz,
    author = "Caprini, Chiara and others",
    title = "{Detecting gravitational waves from cosmological phase transitions with LISA: an update}",
    eprint = "1910.13125",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "DESY-19-159, IPPP/19/27, HIP-2019-14/TH, MITP/19-066, IFT-UAM/CSIC-19-139",
    doi = "10.1088/1475-7516/2020/03/024",
    journal = "JCAP",
    volume = "03",
    pages = "024",
    year = "2020"
}


@article{Caprini:2015zlo,
    author = "Caprini, Chiara and others",
    title = "{Science with the space-based interferometer eLISA. II: Gravitational waves from cosmological phase transitions}",
    eprint = "1512.06239",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "DESY-15-246",
    doi = "10.1088/1475-7516/2016/04/001",
    journal = "JCAP",
    volume = "04",
    pages = "001",
    year = "2016"
}


@article{Kosowsky:1992vn,
    author = "Kosowsky, Arthur and Turner, Michael S.",
    title = "{Gravitational radiation from colliding vacuum bubbles: envelope approximation to many bubble collisions}",
    eprint = "astro-ph/9211004",
    archivePrefix = "arXiv",
    reportNumber = "FERMILAB-PUB-92-295-A",
    doi = "10.1103/PhysRevD.47.4372",
    journal = "Phys. Rev. D",
    volume = "47",
    pages = "4372--4391",
    year = "1993"
}


@article{Huber:2008hg,
    author = "Huber, Stephan J. and Konstandin, Thomas",
    title = "{Gravitational Wave Production by Collisions: More Bubbles}",
    eprint = "0806.1828",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2008/09/022",
    journal = "JCAP",
    volume = "09",
    pages = "022",
    year = "2008"
}


@article{Lewicki:2019gmv,
    author = "Lewicki, Marek and Vaskonen, Ville",
    title = "{On bubble collisions in strongly supercooled phase transitions}",
    eprint = "1912.00997",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "KCL-PH-TH/2019-88",
    doi = "10.1016/j.dark.2020.100672",
    journal = "Phys. Dark Univ.",
    volume = "30",
    pages = "100672",
    year = "2020"
}


@article{Lewicki:2020azd,
    author = "Lewicki, Marek and Vaskonen, Ville",
    title = "{Gravitational waves from colliding vacuum bubbles in gauge theories}",
    eprint = "2012.07826",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1140/epjc/s10052-021-09232-3",
    journal = "Eur. Phys. J. C",
    volume = "81",
    number = "5",
    pages = "437",
    year = "2021",
    note = "[Erratum: Eur.Phys.J.C 81, 1077 (2021)]"
}


@article{Lewicki:2020jiv,
    author = "Lewicki, Marek and Vaskonen, Ville",
    title = "{Gravitational wave spectra from strongly supercooled phase transitions}",
    eprint = "2007.04967",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "KCL-PH-TH/2020-36",
    doi = "10.1140/epjc/s10052-020-08589-1",
    journal = "Eur. Phys. J. C",
    volume = "80",
    number = "11",
    pages = "1003",
    year = "2020"
}


@article{Hindmarsh:2013xza,
    author = "Hindmarsh, Mark and Huber, Stephan J. and Rummukainen, Kari and Weir, David J.",
    title = "{Gravitational waves from the sound of a first order phase transition}",
    eprint = "1304.2433",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "HIP-2013-07-TH",
    doi = "10.1103/PhysRevLett.112.041301",
    journal = "Phys. Rev. Lett.",
    volume = "112",
    pages = "041301",
    year = "2014"
}


@article{Hindmarsh:2015qta,
    author = "Hindmarsh, Mark and Huber, Stephan J. and Rummukainen, Kari and Weir, David J.",
    title = "{Numerical simulations of acoustically generated gravitational waves at a first order phase transition}",
    eprint = "1504.03291",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "HIP-2015-13-TH",
    doi = "10.1103/PhysRevD.92.123009",
    journal = "Phys. Rev. D",
    volume = "92",
    number = "12",
    pages = "123009",
    year = "2015"
}


@article{Hindmarsh:2017gnf,
    author = "Hindmarsh, Mark and Huber, Stephan J. and Rummukainen, Kari and Weir, David J.",
    title = "{Shape of the acoustic gravitational wave power spectrum from a first order phase transition}",
    eprint = "1704.05871",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "HIP-2017-02-TH, HIP-2017-02/TH",
    doi = "10.1103/PhysRevD.96.103520",
    journal = "Phys. Rev. D",
    volume = "96",
    number = "10",
    pages = "103520",
    year = "2017",
    note = "[Erratum: Phys.Rev.D 101, 089902 (2020)]"
}


@article{Hindmarsh:2020hop,
    author = {Hindmarsh, Mark B. and L\"uben, Marvin and Lumma, Johannes and Pauly, Martin},
    title = "{Phase transitions in the early universe}",
    eprint = "2008.09136",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "MPP-2020-163, HIP-2020-27/TH",
    doi = "10.21468/SciPostPhysLectNotes.24",
    journal = "SciPost Phys. Lect. Notes",
    volume = "24",
    pages = "1",
    year = "2021"
}


@article{RoperPol:2019wvy,
    author = "Roper Pol, Alberto and Mandal, Sayan and Brandenburg, Axel and Kahniashvili, Tina and Kosowsky, Arthur",
    title = "{Numerical simulations of gravitational waves from early-universe turbulence}",
    eprint = "1903.08585",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "NORDITA-2019-024",
    doi = "10.1103/PhysRevD.102.083512",
    journal = "Phys. Rev. D",
    volume = "102",
    number = "8",
    pages = "083512",
    year = "2020"
}


@article{Kahniashvili:2020jgm,
    author = "Kahniashvili, Tina and Brandenburg, Axel and Gogoberidze, Grigol and Mandal, Sayan and Roper Pol, Alberto",
    title = "{Circular polarization of gravitational waves from early-Universe helical turbulence}",
    eprint = "2011.05556",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "NORDITA-2020-102",
    doi = "10.1103/PhysRevResearch.3.013193",
    journal = "Phys. Rev. Res.",
    volume = "3",
    number = "1",
    pages = "013193",
    year = "2021"
}


@article{Pol:2021uol,
    author = "Roper Pol, Alberto and Mandal, Sayan and Brandenburg, Axel and Kahniashvili, Tina",
    title = "{Polarization of gravitational waves from helical MHD turbulent sources}",
    eprint = "2107.05356",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    reportNumber = "NORDITA-2021-062",
    doi = "10.1088/1475-7516/2022/04/019",
    journal = "JCAP",
    volume = "04",
    number = "04",
    pages = "019",
    year = "2022"
}


@article{Auclair:2022jod,
    author = "Auclair, Pierre and Caprini, Chiara and Cutting, Daniel and Hindmarsh, Mark and Rummukainen, Kari and Steer, Dani\`ele A. and Weir, David J.",
    title = "{Generation of gravitational waves from freely decaying turbulence}",
    eprint = "2205.02588",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "HIP-2021-35/TH",
    doi = "10.1088/1475-7516/2022/09/029",
    journal = "JCAP",
    volume = "09",
    pages = "029",
    year = "2022"
}


@article{Laurent:2020gpg,
    author = "Laurent, Benoit and Cline, James M.",
    title = "{Fluid equations for fast-moving electroweak bubble walls}",
    eprint = "2007.10935",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.102.063516",
    journal = "Phys. Rev. D",
    volume = "102",
    number = "6",
    pages = "063516",
    year = "2020"
}


@article{Cline:2021iff,
    author = "Cline, James M. and Friedlander, Avi and He, Dong-Ming and Kainulainen, Kimmo and Laurent, Benoit and Tucker-Smith, David",
    title = "{Baryogenesis and gravity waves from a UV-completed electroweak phase transition}",
    eprint = "2102.12490",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.103.123529",
    journal = "Phys. Rev. D",
    volume = "103",
    number = "12",
    pages = "123529",
    year = "2021"
}


@article{Lewicki:2021pgr,
    author = "Lewicki, Marek and Merchand, Marco and Zych, Mateusz",
    title = "{Electroweak bubble wall expansion: gravitational waves and baryogenesis in Standard Model-like thermal plasma}",
    eprint = "2111.02393",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1007/JHEP02(2022)017",
    journal = "JHEP",
    volume = "02",
    pages = "017",
    year = "2022"
}


@article{Laurent:2022jrs,
    author = "Laurent, Benoit and Cline, James M.",
    title = "{First principles determination of bubble wall velocity}",
    eprint = "2204.13120",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.106.023501",
    journal = "Phys. Rev. D",
    volume = "106",
    number = "2",
    pages = "023501",
    year = "2022"
}


@article{Ellis:2022lft,
    author = "Ellis, John and Lewicki, Marek and Merchand, Marco and No, Jos\'e Miguel and Zych, Mateusz",
    title = "{The Scalar Singlet Extension of the Standard Model: Gravitational Waves versus Baryogenesis}",
    eprint = "2210.16305",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    month = "10",
    year = "2022"
}


@article{Espinosa:2010hh,
    author = "Espinosa, Jose R. and Konstandin, Thomas and No, Jose M. and Servant, Geraldine",
    title = "{Energy Budget of Cosmological First-order Phase Transitions}",
    eprint = "1004.4187",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-PH-TH-2010-027",
    doi = "10.1088/1475-7516/2010/06/028",
    journal = "JCAP",
    volume = "06",
    pages = "028",
    year = "2010"
}


@article{Jinno:2019jhi,
    author = "Jinno, Ryusuke and Seong, Hyeonseok and Takimoto, Masahiro and Um, Choong Min",
    title = "{Gravitational waves from first-order phase transitions: Ultra-supercooled transitions and the fate of relativistic shocks}",
    eprint = "1905.00899",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "DESY 19-067, DESY-19-067, CTPU-PTC-19-12, KEK-TH-2125",
    doi = "10.1088/1475-7516/2019/10/033",
    journal = "JCAP",
    volume = "10",
    pages = "033",
    year = "2019"
}


@article{Lewicki:2022pdb,
    author = "Lewicki, Marek and Vaskonen, Ville",
    title = "{Gravitational waves from bubble collisions and fluid motion in strongly supercooled phase transitions}",
    eprint = "2208.11697",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    month = "8",
    year = "2022"
}


@article{Thrane:2013oya,
    author = "Thrane, Eric and Romano, Joseph D.",
    title = "{Sensitivity curves for searches for gravitational-wave backgrounds}",
    eprint = "1310.5300",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    doi = "10.1103/PhysRevD.88.124032",
    journal = "Phys. Rev. D",
    volume = "88",
    number = "12",
    pages = "124032",
    year = "2013"
}


@article{Cui:2019kkd,
    author = "Cui, Yanou and Lewicki, Marek and Morrissey, David E.",
    title = "{Gravitational Wave Bursts as Harbingers of Cosmic Strings Diluted by Inflation}",
    eprint = "1912.08832",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevLett.125.211302",
    journal = "Phys. Rev. Lett.",
    volume = "125",
    number = "21",
    pages = "211302",
    year = "2020"
}


@article{Martins:1995tg,
    author = "Martins, C. J. A. P. and Shellard, E. P. S.",
    title = "{String evolution with friction}",
    eprint = "hep-ph/9507335",
    archivePrefix = "arXiv",
    reportNumber = "DAMTP-R-95-10",
    doi = "10.1103/PhysRevD.53.R575",
    journal = "Phys. Rev. D",
    volume = "53",
    pages = "575--579",
    year = "1996"
}


@article{Martins:1996jp,
    author = "Martins, C. J. A. P. and Shellard, E. P. S.",
    title = "{Quantitative string evolution}",
    eprint = "hep-ph/9602271",
    archivePrefix = "arXiv",
    reportNumber = "DAMTP-R-96-5",
    doi = "10.1103/PhysRevD.54.2535",
    journal = "Phys. Rev. D",
    volume = "54",
    pages = "2535--2556",
    year = "1996"
}


@article{Martins:2000cs,
    author = "Martins, C. J. A. P. and Shellard, E. P. S.",
    title = "{Extending the velocity dependent one scale string evolution model}",
    eprint = "hep-ph/0003298",
    archivePrefix = "arXiv",
    doi = "10.1103/PhysRevD.65.043514",
    journal = "Phys. Rev. D",
    volume = "65",
    pages = "043514",
    year = "2002"
}


@article{Avelino:2012qy,
    author = "Avelino, P. P. and Sousa, L.",
    title = "{Scaling laws for weakly interacting cosmic (super)string and p-brane networks}",
    eprint = "1202.6298",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.85.083525",
    journal = "Phys. Rev. D",
    volume = "85",
    pages = "083525",
    year = "2012"
}


@article{Sousa:2013aaa,
    author = "Sousa, L. and Avelino, P. P.",
    title = "{Stochastic Gravitational Wave Background generated by Cosmic String Networks: Velocity-Dependent One-Scale model versus Scale-Invariant Evolution}",
    eprint = "1304.2445",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.88.023516",
    journal = "Phys. Rev. D",
    volume = "88",
    number = "2",
    pages = "023516",
    year = "2013"
}


@book{Vilenkin:2000jqa,
    author = "Vilenkin, A. and Shellard, E. P. S.",
    title = "{Cosmic Strings and Other Topological Defects}",
    isbn = "978-0-521-65476-0",
    publisher = "Cambridge University Press",
    month = "7",
    year = "2000"
}


==> refs.tex <==
%\cite{Caprini:2018mtu}
\bibitem{Caprini:2018mtu}
C.~Caprini and D.~G.~Figueroa,
%``Cosmological Backgrounds of Gravitational Waves,''
Class. Quant. Grav. \textbf{35}, no.16, 163001 (2018)
doi:10.1088/1361-6382/aac608
[arXiv:1801.04268 [astro-ph.CO]].
%426 citations counted in INSPIRE as of 16 Sep 2022



%\cite{Giovannini:1998bp}
\bibitem{Giovannini:1998bp}
M.~Giovannini,
%``Gravitational waves constraints on postinflationary phases stiffer than radiation,''
Phys. Rev. D \textbf{58}, 083504 (1998)
doi:10.1103/PhysRevD.58.083504
[arXiv:hep-ph/9806329 [hep-ph]].
%130 citations counted in INSPIRE as of 26 Aug 2022

%\cite{Giovannini:2009kg}
\bibitem{Giovannini:2009kg}
M.~Giovannini,
%``Stochastic backgrounds of relic gravitons: a theoretical appraisal,''
PMC Phys. A \textbf{4}, 1 (2010)
doi:10.1186/1754-0410-4-1
[arXiv:0901.3026 [astro-ph.CO]].
%43 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Riazuelo:2000fc}
\bibitem{Riazuelo:2000fc}
A.~Riazuelo and J.~P.~Uzan,
%``Quintessence and gravitational waves,''
Phys. Rev. D \textbf{62}, 083506 (2000)
doi:10.1103/PhysRevD.62.083506
[arXiv:astro-ph/0004156 [astro-ph]].
%111 citations counted in INSPIRE as of 07 Sep 2022

%\cite{Sahni:2001qp}
\bibitem{Sahni:2001qp}
V.~Sahni, M.~Sami and T.~Souradeep,
%``Relic gravity waves from brane world inflation,''
Phys. Rev. D \textbf{65}, 023518 (2002)
doi:10.1103/PhysRevD.65.023518
[arXiv:gr-qc/0105121 [gr-qc]].
%215 citations counted in INSPIRE as of 19 Aug 2022

%\cite{Seto:2003kc}
\bibitem{Seto:2003kc}
N.~Seto and J.~Yokoyama,
%``Probing the equation of state of the early universe with a space laser interferometer,''
J. Phys. Soc. Jap. \textbf{72}, 3082-3086 (2003)
doi:10.1143/JPSJ.72.3082
[arXiv:gr-qc/0305096 [gr-qc]].
%83 citations counted in INSPIRE as of 23 Aug 2022

%\cite{Tashiro:2003qp}
\bibitem{Tashiro:2003qp}
H.~Tashiro, T.~Chiba and M.~Sasaki,
%``Reheating after quintessential inflation and gravitational waves,''
Class. Quant. Grav. \textbf{21}, 1761-1772 (2004)
doi:10.1088/0264-9381/21/7/004
[arXiv:gr-qc/0307068 [gr-qc]].
%111 citations counted in INSPIRE as of 18 Aug 2022

%\cite{Nakayama:2008ip}
\bibitem{Nakayama:2008ip}
K.~Nakayama, S.~Saito, Y.~Suwa and J.~Yokoyama,
%``Space laser interferometers can determine the thermal history of the early Universe,''
Phys. Rev. D \textbf{77}, 124001 (2008)
doi:10.1103/PhysRevD.77.124001
[arXiv:0802.2452 [hep-ph]].
%75 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Nakayama:2008wy}
\bibitem{Nakayama:2008wy}
K.~Nakayama, S.~Saito, Y.~Suwa and J.~Yokoyama,
%``Probing reheating temperature of the universe with gravitational wave background,''
JCAP \textbf{06}, 020 (2008)
doi:10.1088/1475-7516/2008/06/020
[arXiv:0804.1827 [astro-ph]].
%116 citations counted in INSPIRE as of 23 Aug 2022

%\cite{Durrer:2011bi}
\bibitem{Durrer:2011bi}
R.~Durrer and J.~Hasenkamp,
%``Testing Superstring Theories with Gravitational Waves,''
Phys. Rev. D \textbf{84}, 064027 (2011)
doi:10.1103/PhysRevD.84.064027
[arXiv:1105.5283 [gr-qc]].
%27 citations counted in INSPIRE as of 13 Sep 2022

%\cite{Kuroyanagi:2011fy}
\bibitem{Kuroyanagi:2011fy}
S.~Kuroyanagi, K.~Nakayama and S.~Saito,
%``Prospects for determination of thermal history after inflation with future gravitational wave detectors,''
Phys. Rev. D \textbf{84}, 123513 (2011)
doi:10.1103/PhysRevD.84.123513
[arXiv:1110.4169 [astro-ph.CO]].
%53 citations counted in INSPIRE as of 26 Aug 2022

%\cite{Kuroyanagi:2018csn}
\bibitem{Kuroyanagi:2018csn}
S.~Kuroyanagi, T.~Chiba and T.~Takahashi,
%``Probing the Universe through the Stochastic Gravitational Wave Background,''
JCAP \textbf{11}, 038 (2018)
doi:10.1088/1475-7516/2018/11/038
[arXiv:1807.00786 [astro-ph.CO]].
%60 citations counted in INSPIRE as of 16 Sep 2022

%\cite{Jinno:2012xb}
\bibitem{Jinno:2012xb}
R.~Jinno, T.~Moroi and K.~Nakayama,
%``Probing dark radiation with inflationary gravitational waves,''
Phys. Rev. D \textbf{86}, 123502 (2012)
doi:10.1103/PhysRevD.86.123502
[arXiv:1208.0184 [astro-ph.CO]].
%24 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Lasky:2015lej}
\bibitem{Lasky:2015lej}
P.~D.~Lasky, C.~M.~F.~Mingarelli, T.~L.~Smith, J.~T.~Giblin, D.~J.~Reardon, R.~Caldwell, M.~Bailes, N.~D.~R.~Bhat, S.~Burke-Spolaor and W.~Coles, \textit{et al.}
%``Gravitational-wave cosmology across 29 decades in frequency,''
Phys. Rev. X \textbf{6}, no.1, 011035 (2016)
doi:10.1103/PhysRevX.6.011035
[arXiv:1511.05994 [astro-ph.CO]].
%162 citations counted in INSPIRE as of 13 Sep 2022

%\cite{Li:2016mmc}
\bibitem{Li:2016mmc}
B.~Li, P.~R.~Shapiro and T.~Rindler-Daller,
%``Bose-Einstein-condensed scalar field dark matter and the gravitational wave background from inflation: new cosmological constraints and its detectability by LIGO,''
Phys. Rev. D \textbf{96}, no.6, 063505 (2017)
doi:10.1103/PhysRevD.96.063505
[arXiv:1611.07961 [astro-ph.CO]].
%45 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Saikawa:2018rcs}
\bibitem{Saikawa:2018rcs}
K.~Saikawa and S.~Shirai,
%``Primordial gravitational waves, precisely: The role of thermodynamics in the Standard Model,''
JCAP \textbf{05}, 035 (2018)
doi:10.1088/1475-7516/2018/05/035
[arXiv:1803.01038 [hep-ph]].
%106 citations counted in INSPIRE as of 16 Sep 2022

%\cite{Caldwell:2018giq}
\bibitem{Caldwell:2018giq}
R.~R.~Caldwell, T.~L.~Smith and D.~G.~E.~Walker,
%``Using a Primordial Gravitational Wave Background to Illuminate New Physics,''
Phys. Rev. D \textbf{100}, no.4, 043513 (2019)
doi:10.1103/PhysRevD.100.043513
[arXiv:1812.07577 [astro-ph.CO]].
%35 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Bernal:2019lpc}
\bibitem{Bernal:2019lpc}
N.~Bernal and F.~Hajkarim,
%``Primordial Gravitational Waves in Nonstandard Cosmologies,''
Phys. Rev. D \textbf{100}, no.6, 063502 (2019)
doi:10.1103/PhysRevD.100.063502
[arXiv:1905.10410 [astro-ph.CO]].
%48 citations counted in INSPIRE as of 16 Sep 2022

%\cite{Figueroa:2019paj}
\bibitem{Figueroa:2019paj}
D.~G.~Figueroa and E.~H.~Tanin,
%``Ability of LIGO and LISA to probe the equation of state of the early Universe,''
JCAP \textbf{08}, 011 (2019)
doi:10.1088/1475-7516/2019/08/011
[arXiv:1905.11960 [astro-ph.CO]].
%48 citations counted in INSPIRE as of 16 Sep 2022

%\cite{DEramo:2019tit}
\bibitem{DEramo:2019tit}
F.~D'Eramo and K.~Schmitz,
%``Imprint of a scalar era on the primordial spectrum of gravitational waves,''
Phys. Rev. Research. \textbf{1}, 013010 (2019)
doi:10.1103/PhysRevResearch.1.013010
[arXiv:1904.07870 [hep-ph]].
%35 citations counted in INSPIRE as of 16 Sep 2022

%\cite{Cui:2017ufi}
\bibitem{Cui:2017ufi}
Y.~Cui, M.~Lewicki, D.~E.~Morrissey and J.~D.~Wells,
%``Cosmic Archaeology with Gravitational Waves from Cosmic Strings,''
Phys. Rev. D \textbf{97}, no.12, 123505 (2018)
doi:10.1103/PhysRevD.97.123505
[arXiv:1711.03104 [hep-ph]].
%83 citations counted in INSPIRE as of 16 Sep 2022

%\cite{Cui:2018rwi}
\bibitem{Cui:2018rwi}
Y.~Cui, M.~Lewicki, D.~E.~Morrissey and J.~D.~Wells,
%``Probing the pre-BBN universe with gravitational waves from cosmic strings,''
JHEP \textbf{01}, 081 (2019)
doi:10.1007/JHEP01(2019)081
[arXiv:1808.08968 [hep-ph]].
%92 citations counted in INSPIRE as of 16 Sep 2022

%\cite{Auclair:2019wcv}
\bibitem{Auclair:2019wcv}
P.~Auclair, J.~J.~Blanco-Pillado, D.~G.~Figueroa, A.~C.~Jenkins, M.~Lewicki, M.~Sakellariadou, S.~Sanidas, L.~Sousa, D.~A.~Steer and J.~M.~Wachter, \textit{et al.}
%``Probing the gravitational wave background from cosmic strings with LISA,''
JCAP \textbf{04}, 034 (2020)
doi:10.1088/1475-7516/2020/04/034
[arXiv:1909.00819 [astro-ph.CO]].
%137 citations counted in INSPIRE as of 16 Sep 2022

%\cite{Guedes:2018afo}
\bibitem{Guedes:2018afo}
G.~S.~F.~Guedes, P.~P.~Avelino and L.~Sousa,
%``Signature of inflation in the stochastic gravitational wave background generated by cosmic string networks,''
Phys. Rev. D \textbf{98}, no.12, 123505 (2018)
doi:10.1103/PhysRevD.98.123505
[arXiv:1809.10802 [astro-ph.CO]].
%25 citations counted in INSPIRE as of 16 Sep 2022

%\cite{Ramberg:2019dgi}
\bibitem{Ramberg:2019dgi}
N.~Ramberg and L.~Visinelli,
%``Probing the Early Universe with Axion Physics and Gravitational Waves,''
Phys. Rev. D \textbf{99}, no.12, 123513 (2019)
doi:10.1103/PhysRevD.99.123513
[arXiv:1904.05707 [astro-ph.CO]].
%40 citations counted in INSPIRE as of 22 Aug 2022

%\cite{Chang:2019mza}
\bibitem{Chang:2019mza}
C.~F.~Chang and Y.~Cui,
%``Stochastic Gravitational Wave Background from Global Cosmic Strings,''
Phys. Dark Univ. \textbf{29}, 100604 (2020)
doi:10.1016/j.dark.2020.100604
[arXiv:1910.04781 [hep-ph]].
%32 citations counted in INSPIRE as of 16 Sep 2022

%\cite{Vilenkin:1981bx}
\bibitem{Vilenkin:1981bx}
A.~Vilenkin,
%``Gravitational radiation from cosmic strings,''
Phys. Lett. B \textbf{107}, 47-50 (1981)
doi:10.1016/0370-2693(81)91144-8
%248 citations counted in INSPIRE as of 05 Sep 2022

%\cite{Hogan:1984is}
\bibitem{Hogan:1984is}
C.~J.~Hogan and M.~J.~Rees,
%``Gravitational interactions of cosmic strings,''
Nature \textbf{311}, 109-113 (1984)
doi:10.1038/311109a0
%178 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Vachaspati:1984gt}
\bibitem{Vachaspati:1984gt}
T.~Vachaspati and A.~Vilenkin,
%``Gravitational Radiation from Cosmic Strings,''
Phys. Rev. D \textbf{31}, 3052 (1985)
doi:10.1103/PhysRevD.31.3052
%462 citations counted in INSPIRE as of 13 Sep 2022

%\cite{Accetta:1988bg}
\bibitem{Accetta:1988bg}
F.~S.~Accetta and L.~M.~Krauss,
%``The stochastic gravitational wave spectrum resulting from cosmic string evolution,''
Nucl. Phys. B \textbf{319}, 747-764 (1989)
doi:10.1016/0550-3213(89)90628-7
%52 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Bennett:1990ry}
\bibitem{Bennett:1990ry}
D.~P.~Bennett and F.~R.~Bouchet,
%``Constraints on the gravity wave background generated by cosmic strings,''
Phys. Rev. D \textbf{43}, 2733-2735 (1991)
doi:10.1103/PhysRevD.43.2733
%42 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Caldwell:1991jj}
\bibitem{Caldwell:1991jj}
R.~R.~Caldwell and B.~Allen,
%``Cosmological constraints on cosmic string gravitational radiation,''
Phys. Rev. D \textbf{45}, 3447-3468 (1992)
doi:10.1103/PhysRevD.45.3447
%190 citations counted in INSPIRE as of 07 Sep 2022

%\cite{Allen:1991bk}
\bibitem{Allen:1991bk}
B.~Allen and E.~P.~S.~Shellard,
%``Gravitational radiation from cosmic strings,''
Phys. Rev. D \textbf{45}, 1898-1912 (1992)
doi:10.1103/PhysRevD.45.1898
%77 citations counted in INSPIRE as of 05 Sep 2022

%\cite{Battye:1997ji}
\bibitem{Battye:1997ji}
R.~A.~Battye, R.~R.~Caldwell and E.~P.~S.~Shellard,
%``Gravitational waves from cosmic strings,''
[arXiv:astro-ph/9706013 [astro-ph]].
%29 citations counted in INSPIRE as of 11 Aug 2022

%\cite{DePies:2007bm}
\bibitem{DePies:2007bm}
M.~R.~DePies and C.~J.~Hogan,
%``Stochastic Gravitational Wave Background from Light Cosmic Strings,''
Phys. Rev. D \textbf{75}, 125006 (2007)
doi:10.1103/PhysRevD.75.125006
[arXiv:astro-ph/0702335 [astro-ph]].
%97 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Siemens:2006yp}
\bibitem{Siemens:2006yp}
X.~Siemens, V.~Mandic and J.~Creighton,
%``Gravitational wave stochastic background from cosmic (super)strings,''
Phys. Rev. Lett. \textbf{98}, 111101 (2007)
doi:10.1103/PhysRevLett.98.111101
[arXiv:astro-ph/0610920 [astro-ph]].
%240 citations counted in INSPIRE as of 16 Sep 2022

%\cite{Olmez:2010bi}
\bibitem{Olmez:2010bi}
S.~Olmez, V.~Mandic and X.~Siemens,
%``Gravitational-Wave Stochastic Background from Kinks and Cusps on Cosmic Strings,''
Phys. Rev. D \textbf{81}, 104028 (2010)
doi:10.1103/PhysRevD.81.104028
[arXiv:1004.0890 [astro-ph.CO]].
%197 citations counted in INSPIRE as of 07 Sep 2022

%\cite{Regimbau:2011bm}
\bibitem{Regimbau:2011bm}
T.~Regimbau, S.~Giampanis, X.~Siemens and V.~Mandic,
%``The stochastic background from cosmic (super)strings: popcorn and (Gaussian) continuous regimes,''
Phys. Rev. D \textbf{85}, 066001 (2012)
doi:10.1103/PhysRevD.85.066001
[arXiv:1111.6638 [astro-ph.CO]].
%34 citations counted in INSPIRE as of 07 Sep 2022

%\cite{Sanidas:2012ee}
\bibitem{Sanidas:2012ee}
S.~A.~Sanidas, R.~A.~Battye and B.~W.~Stappers,
%``Constraints on cosmic string tension imposed by the limit on the stochastic gravitational wave background from the European Pulsar Timing Array,''
Phys. Rev. D \textbf{85}, 122003 (2012)
doi:10.1103/PhysRevD.85.122003
[arXiv:1201.2419 [astro-ph.CO]].
%134 citations counted in INSPIRE as of 05 Sep 2022

%\cite{Sanidas:2012tf}
\bibitem{Sanidas:2012tf}
S.~A.~Sanidas, R.~A.~Battye and B.~W.~Stappers,
%``Projected constraints on the cosmic (super)string tension with future gravitational wave detection experiments,''
Astrophys. J. \textbf{764}, 108 (2013)
doi:10.1088/0004-637X/764/1/108
[arXiv:1211.5042 [astro-ph.CO]].
%34 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Binetruy:2012ze}
\bibitem{Binetruy:2012ze}
P.~Binetruy, A.~Bohe, C.~Caprini and J.~F.~Dufaux,
%``Cosmological Backgrounds of Gravitational Waves and eLISA/NGO: Phase Transitions, Cosmic Strings and Other Sources,''
JCAP \textbf{06}, 027 (2012)
doi:10.1088/1475-7516/2012/06/027
[arXiv:1201.0983 [gr-qc]].
%257 citations counted in INSPIRE as of 05 Sep 2022

%\cite{Kuroyanagi:2012wm}
\bibitem{Kuroyanagi:2012wm}
S.~Kuroyanagi, K.~Miyamoto, T.~Sekiguchi, K.~Takahashi and J.~Silk,
%``Forecast constraints on cosmic string parameters from gravitational wave direct detection experiments,''
Phys. Rev. D \textbf{86}, 023503 (2012)
doi:10.1103/PhysRevD.86.023503
[arXiv:1202.3032 [astro-ph.CO]].
%56 citations counted in INSPIRE as of 05 Sep 2022

%\cite{Kuroyanagi:2012jf}
\bibitem{Kuroyanagi:2012jf}
S.~Kuroyanagi, K.~Miyamoto, T.~Sekiguchi, K.~Takahashi and J.~Silk,
%``Forecast constraints on cosmic strings from future CMB, pulsar timing and gravitational wave direct detection experiments,''
Phys. Rev. D \textbf{87}, no.2, 023522 (2013)
[erratum: Phys. Rev. D \textbf{87}, no.6, 069903 (2013)]
doi:10.1103/PhysRevD.87.023522
[arXiv:1210.2829 [astro-ph.CO]].
%46 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Sousa:2016ggw}
\bibitem{Sousa:2016ggw}
L.~Sousa and P.~P.~Avelino,
%``Probing Cosmic Superstrings with Gravitational Waves,''
Phys. Rev. D \textbf{94}, no.6, 063529 (2016)
doi:10.1103/PhysRevD.94.063529
[arXiv:1606.05585 [astro-ph.CO]].
%37 citations counted in INSPIRE as of 05 Sep 2022

%\cite{Sousa:2020sxs}
\bibitem{Sousa:2020sxs}
L.~Sousa, P.~P.~Avelino and G.~S.~F.~Guedes,
%``Full analytical approximation to the stochastic gravitational wave background generated by cosmic string networks,''
Phys. Rev. D \textbf{101}, no.10, 103508 (2020)
doi:10.1103/PhysRevD.101.103508
[arXiv:2002.01079 [astro-ph.CO]].
%21 citations counted in INSPIRE as of 16 Sep 2022

%\cite{Spokoiny:1993kt}
\bibitem{Spokoiny:1993kt}
B.~Spokoiny,
%``Deflationary universe scenario,''
Phys. Lett. B \textbf{315}, 40-45 (1993)
doi:10.1016/0370-2693(93)90155-B
[arXiv:gr-qc/9306008 [gr-qc]].
%266 citations counted in INSPIRE as of 07 Sep 2022

%\cite{Joyce:1996cp}
\bibitem{Joyce:1996cp}
M.~Joyce,
%``Electroweak Baryogenesis and the Expansion Rate of the Universe,''
Phys. Rev. D \textbf{55}, 1875-1878 (1997)
doi:10.1103/PhysRevD.55.1875
[arXiv:hep-ph/9606223 [hep-ph]].
%178 citations counted in INSPIRE as of 09 Sep 2022

%\cite{Creminelli:2001th}
\bibitem{Creminelli:2001th}
P.~Creminelli, A.~Nicolis and R.~Rattazzi,
%``Holography and the electroweak phase transition,''
JHEP \textbf{03}, 051 (2002)
doi:10.1088/1126-6708/2002/03/051
[arXiv:hep-th/0107141 [hep-th]].
%136 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Randall:2006py}
\bibitem{Randall:2006py}
L.~Randall and G.~Servant,
%``Gravitational waves from warped spacetime,''
JHEP \textbf{05}, 054 (2007)
doi:10.1088/1126-6708/2007/05/054
[arXiv:hep-ph/0607158 [hep-ph]].
%157 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Nardini:2007me}
\bibitem{Nardini:2007me}
G.~Nardini, M.~Quiros and A.~Wulzer,
%``A Confining Strong First-Order Electroweak Phase Transition,''
JHEP \textbf{09}, 077 (2007)
doi:10.1088/1126-6708/2007/09/077
[arXiv:0706.3388 [hep-ph]].
%83 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Konstandin:2011dr}
\bibitem{Konstandin:2011dr}
T.~Konstandin and G.~Servant,
%``Cosmological Consequences of Nearly Conformal Dynamics at the TeV scale,''
JCAP \textbf{12}, 009 (2011)
doi:10.1088/1475-7516/2011/12/009
[arXiv:1104.4791 [hep-ph]].
%119 citations counted in INSPIRE as of 11 Aug 2022

%\cite{vonHarling:2017yew}
\bibitem{vonHarling:2017yew}
B.~von Harling and G.~Servant,
%``QCD-induced Electroweak Phase Transition,''
JHEP \textbf{01}, 159 (2018)
doi:10.1007/JHEP01(2018)159
[arXiv:1711.11554 [hep-ph]].
%76 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Iso:2017uuu}
\bibitem{Iso:2017uuu}
S.~Iso, P.~D.~Serpico and K.~Shimada,
%``QCD-Electroweak First-Order Phase Transition in a Supercooled Universe,''
Phys. Rev. Lett. \textbf{119}, no.14, 141301 (2017)
doi:10.1103/PhysRevLett.119.141301
[arXiv:1704.04955 [hep-ph]].
%84 citations counted in INSPIRE as of 25 Aug 2022

%\cite{Bruggisser:2018mrt}
\bibitem{Bruggisser:2018mrt}
S.~Bruggisser, B.~Von Harling, O.~Matsedonskyi and G.~Servant,
%``Electroweak Phase Transition and Baryogenesis in Composite Higgs Models,''
JHEP \textbf{12}, 099 (2018)
doi:10.1007/JHEP12(2018)099
[arXiv:1804.07314 [hep-ph]].
%113 citations counted in INSPIRE as of 07 Sep 2022

%\cite{Baratella:2018pxi}
\bibitem{Baratella:2018pxi}
P.~Baratella, A.~Pomarol and F.~Rompineve,
%``The Supercooled Universe,''
JHEP \textbf{03}, 100 (2019)
doi:10.1007/JHEP03(2019)100
[arXiv:1812.06996 [hep-ph]].
%65 citations counted in INSPIRE as of 25 Aug 2022

%\cite{Agashe:2019lhy}
\bibitem{Agashe:2019lhy}
K.~Agashe, P.~Du, M.~Ekhterachian, S.~Kumar and R.~Sundrum,
%``Cosmological Phase Transition of Spontaneous Confinement,''
JHEP \textbf{05}, 086 (2020)
doi:10.1007/JHEP05(2020)086
[arXiv:1910.06238 [hep-ph]].
%31 citations counted in INSPIRE as of 23 Aug 2022

%\cite{DelleRose:2019pgi}
\bibitem{DelleRose:2019pgi}
L.~Delle Rose, G.~Panico, M.~Redi and A.~Tesi,
%``Gravitational Waves from Supercool Axions,''
JHEP \textbf{04}, 025 (2020)
doi:10.1007/JHEP04(2020)025
[arXiv:1912.06139 [hep-ph]].
%51 citations counted in INSPIRE as of 16 Sep 2022

%\cite{vonHarling:2019gme}
\bibitem{vonHarling:2019gme}
B.~Von Harling, A.~Pomarol, O.~Pujol\`as and F.~Rompineve,
%``Peccei-Quinn Phase Transition at LIGO,''
JHEP \textbf{04}, 195 (2020)
doi:10.1007/JHEP04(2020)195
[arXiv:1912.07587 [hep-ph]].
%54 citations counted in INSPIRE as of 16 Sep 2022

%\cite{Espinosa:2010hh}
\bibitem{Espinosa:2010hh}
J.~R.~Espinosa, T.~Konstandin, J.~M.~No and G.~Servant,
%``Energy Budget of Cosmological First-order Phase Transitions,''
JCAP \textbf{06}, 028 (2010)
doi:10.1088/1475-7516/2010/06/028
[arXiv:1004.4187 [hep-ph]].
%345 citations counted in INSPIRE as of 15 Sep 2022


%\cite{Ellis:2019oqb}
\bibitem{Ellis:2019oqb}
J.~Ellis, M.~Lewicki, J.~M.~No and V.~Vaskonen,
%``Gravitational wave energy budget in strongly supercooled phase transitions,''
JCAP \textbf{06}, 024 (2019)
doi:10.1088/1475-7516/2019/06/024
[arXiv:1903.09642 [hep-ph]].
%159 citations counted in INSPIRE as of 18 Sep 2022

%\cite{Cutting:2018tjt}
\bibitem{Cutting:2018tjt}
D.~Cutting, M.~Hindmarsh and D.~J.~Weir,
%``Gravitational waves from vacuum first-order phase transitions: from the envelope to the lattice,''
Phys. Rev. D \textbf{97}, no.12, 123513 (2018)
doi:10.1103/PhysRevD.97.123513
[arXiv:1802.05712 [astro-ph.CO]].
%117 citations counted in INSPIRE as of 12 Sep 2022

%\cite{Hindmarsh:2013xza}
\bibitem{Hindmarsh:2013xza}
M.~Hindmarsh, S.~J.~Huber, K.~Rummukainen and D.~J.~Weir,
%``Gravitational waves from the sound of a first order phase transition,''
Phys. Rev. Lett. \textbf{112}, 041301 (2014)
doi:10.1103/PhysRevLett.112.041301
[arXiv:1304.2433 [hep-ph]].
%310 citations counted in INSPIRE as of 13 Sep 2022

%\cite{Hindmarsh:2015qta}
\bibitem{Hindmarsh:2015qta}
M.~Hindmarsh, S.~J.~Huber, K.~Rummukainen and D.~J.~Weir,
%``Numerical simulations of acoustically generated gravitational waves at a first order phase transition,''
Phys. Rev. D \textbf{92}, no.12, 123009 (2015)
doi:10.1103/PhysRevD.92.123009
[arXiv:1504.03291 [astro-ph.CO]].
%309 citations counted in INSPIRE as of 12 Sep 2022

%\cite{Hindmarsh:2016lnk}
\bibitem{Hindmarsh:2016lnk}
M.~Hindmarsh,
%``Sound shell model for acoustic gravitational wave production at a first-order phase transition in the early Universe,''
Phys. Rev. Lett. \textbf{120}, no.7, 071301 (2018)
doi:10.1103/PhysRevLett.120.071301
[arXiv:1608.04735 [astro-ph.CO]].
%90 citations counted in INSPIRE as of 12 Sep 2022

%\cite{Hindmarsh:2017gnf}
\bibitem{Hindmarsh:2017gnf}
M.~Hindmarsh, S.~J.~Huber, K.~Rummukainen and D.~J.~Weir,
%``Shape of the acoustic gravitational wave power spectrum from a first order phase transition,''
Phys. Rev. D \textbf{96}, no.10, 103520 (2017)
[erratum: Phys. Rev. D \textbf{101}, no.8, 089902 (2020)]
doi:10.1103/PhysRevD.96.103520
[arXiv:1704.05871 [astro-ph.CO]].
%215 citations counted in INSPIRE as of 12 Sep 2022

%\cite{Caprini:2015zlo}
\bibitem{Caprini:2015zlo}
C.~Caprini, M.~Hindmarsh, S.~Huber, T.~Konstandin, J.~Kozaczuk, G.~Nardini, J.~M.~No, A.~Petiteau, P.~Schwaller and G.~Servant, \textit{et al.}
%``Science with the space-based interferometer eLISA. II: Gravitational waves from cosmological phase transitions,''
JCAP \textbf{04}, 001 (2016)
doi:10.1088/1475-7516/2016/04/001
[arXiv:1512.06239 [astro-ph.CO]].
%610 citations counted in INSPIRE as of 15 Sep 2022

%\cite{Ellis:2018mja}
\bibitem{Ellis:2018mja}
J.~Ellis, M.~Lewicki and J.~M.~No,
%``On the Maximal Strength of a First-Order Electroweak Phase Transition and its Gravitational Wave Signal,''
JCAP \textbf{04}, 003 (2019)
doi:10.1088/1475-7516/2019/04/003
[arXiv:1809.08242 [hep-ph]].
%192 citations counted in INSPIRE as of 01 Sep 2022

%\cite{Bodeker:2017cim}
\bibitem{Bodeker:2017cim}
D.~Bodeker and G.~D.~Moore,
%``Electroweak Bubble Wall Speed Limit,''
JCAP \textbf{05}, 025 (2017)
doi:10.1088/1475-7516/2017/05/025
[arXiv:1703.08215 [hep-ph]].
%162 citations counted in INSPIRE as of 15 Sep 2022

%\cite{Caprini:2009yp}
\bibitem{Caprini:2009yp}
C.~Caprini, R.~Durrer and G.~Servant,
%``The stochastic gravitational wave background from turbulence and magnetic fields generated by a first-order phase transition,''
JCAP \textbf{12}, 024 (2009)
doi:10.1088/1475-7516/2009/12/024
[arXiv:0909.0622 [astro-ph.CO]].
%320 citations counted in INSPIRE as of 13 Sep 2022

%\cite{Gogoberidze:2007an}
\bibitem{Gogoberidze:2007an}
G.~Gogoberidze, T.~Kahniashvili and A.~Kosowsky,
%``The Spectrum of Gravitational Radiation from Primordial Turbulence,''
Phys. Rev. D \textbf{76}, 083002 (2007)
doi:10.1103/PhysRevD.76.083002
[arXiv:0705.1733 [astro-ph]].
%142 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Niksa:2018ofa}
\bibitem{Niksa:2018ofa}
P.~Niksa, M.~Schlederer and G.~Sigl,
%``Gravitational Waves produced by Compressible MHD Turbulence from Cosmological Phase Transitions,''
Class. Quant. Grav. \textbf{35}, no.14, 144001 (2018)
doi:10.1088/1361-6382/aac89c
[arXiv:1803.02271 [astro-ph.CO]].
%60 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Pol:2019yex}
\bibitem{Pol:2019yex}
A.~Roper Pol, S.~Mandal, A.~Brandenburg, T.~Kahniashvili and A.~Kosowsky,
%``Numerical simulations of gravitational waves from early-universe turbulence,''
Phys. Rev. D \textbf{102}, no.8, 083512 (2020)
doi:10.1103/PhysRevD.102.083512
[arXiv:1903.08585 [astro-ph.CO]].
%75 citations counted in INSPIRE as of 01 Sep 2022

%\cite{Child:2012qg}
\bibitem{Child:2012qg}
H.~L.~Child and J.~T.~Giblin, Jr.,
%``Gravitational Radiation from First-Order Phase Transitions,''
JCAP \textbf{10}, 001 (2012)
doi:10.1088/1475-7516/2012/10/001
[arXiv:1207.6408 [astro-ph.CO]].
%42 citations counted in INSPIRE as of 16 Aug 2022

%\cite{Fairbairn:2019xog}
\bibitem{Fairbairn:2019xog}
M.~Fairbairn, E.~Hardy and A.~Wickens,
%``Hearing without seeing: gravitational waves from hot and cold hidden sectors,''
JHEP \textbf{07}, 044 (2019)
doi:10.1007/JHEP07(2019)044
[arXiv:1901.11038 [hep-ph]].
%50 citations counted in INSPIRE as of 25 Aug 2022

%\cite{Cui:2019kkd}
\bibitem{Cui:2019kkd}
Y.~Cui, M.~Lewicki and D.~E.~Morrissey,
%``Gravitational Wave Bursts as Harbingers of Cosmic Strings Diluted by Inflation,''
Phys. Rev. Lett. \textbf{125}, no.21, 211302 (2020)
doi:10.1103/PhysRevLett.125.211302
[arXiv:1912.08832 [hep-ph]].
%31 citations counted in INSPIRE as of 18 Sep 2022

%\cite{Martins:1995tg}
\bibitem{Martins:1995tg}
C.~J.~A.~P.~Martins and E.~P.~S.~Shellard,
%``String evolution with friction,''
Phys. Rev. D \textbf{53}, 575-579 (1996)
doi:10.1103/PhysRevD.53.R575
[arXiv:hep-ph/9507335 [hep-ph]].
%96 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Martins:1996jp}
\bibitem{Martins:1996jp}
C.~J.~A.~P.~Martins and E.~P.~S.~Shellard,
%``Quantitative string evolution,''
Phys. Rev. D \textbf{54}, 2535-2556 (1996)
doi:10.1103/PhysRevD.54.2535
[arXiv:hep-ph/9602271 [hep-ph]].
%255 citations counted in INSPIRE as of 05 Sep 2022

%\cite{Martins:2000cs}
\bibitem{Martins:2000cs}
C.~J.~A.~P.~Martins and E.~P.~S.~Shellard,
%``Extending the velocity dependent one scale string evolution model,''
Phys. Rev. D \textbf{65}, 043514 (2002)
doi:10.1103/PhysRevD.65.043514
[arXiv:hep-ph/0003298 [hep-ph]].
%214 citations counted in INSPIRE as of 05 Sep 2022

%\cite{Avelino:2012qy}
\bibitem{Avelino:2012qy}
P.~P.~Avelino and L.~Sousa,
%``Scaling laws for weakly interacting cosmic (super)string and p-brane networks,''
Phys. Rev. D \textbf{85}, 083525 (2012)
doi:10.1103/PhysRevD.85.083525
[arXiv:1202.6298 [astro-ph.CO]].
%13 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Sousa:2013aaa}
\bibitem{Sousa:2013aaa}
L.~Sousa and P.~P.~Avelino,
%``Stochastic Gravitational Wave Background generated by Cosmic String Networks: Velocity-Dependent One-Scale model versus Scale-Invariant Evolution,''
Phys. Rev. D \textbf{88}, no.2, 023516 (2013)
doi:10.1103/PhysRevD.88.023516
[arXiv:1304.2445 [astro-ph.CO]].
%37 citations counted in INSPIRE as of 18 Aug 2022

%\cite{Akrami:2018odb}
\bibitem{Akrami:2018odb}
Y.~Akrami \textit{et al.} [Planck],
%``Planck 2018 results. X. Constraints on inflation,''
Astron. Astrophys. \textbf{641}, A10 (2020)
doi:10.1051/0004-6361/201833887
[arXiv:1807.06211 [astro-ph.CO]].
%2022 citations counted in INSPIRE as of 16 Sep 2022

%\cite{Vilenkin:2000jqa}
\bibitem{Vilenkin:2000jqa}
A.~Vilenkin and E.~P.~S.~Shellard,
%``Cosmic Strings and Other Topological Defects,''
Cambridge University Press, 2000,
ISBN 978-0-521-65476-0
%60 citations counted in INSPIRE as of 15 Sep 2022

%\cite{Guth:1979bh}
\bibitem{Guth:1979bh}
A.~H.~Guth and S.~H.~H.~Tye,
%``Phase Transitions and Magnetic Monopole Production in the Very Early Universe,''
Phys. Rev. Lett. \textbf{44}, 631 (1980)
[erratum: Phys. Rev. Lett. \textbf{44}, 963 (1980)]
doi:10.1103/PhysRevLett.44.631
%343 citations counted in INSPIRE as of 08 Sep 2022

%\cite{Guth:1981uk}
\bibitem{Guth:1981uk}
A.~H.~Guth and E.~J.~Weinberg,
%``Cosmological Consequences of a First Order Phase Transition in the SU(5) Grand Unified Model,''
Phys. Rev. D \textbf{23}, 876 (1981)
doi:10.1103/PhysRevD.23.876
%310 citations counted in INSPIRE as of 11 Aug 2022

%\cite{Kolb:1990vq}
\bibitem{Kolb:1990vq}
E.~W.~Kolb and M.~S.~Turner,
%``The Early Universe,''
Front. Phys. \textbf{69}, 1-547 (1990)
doi:10.1201/9780429492860
%2026 citations counted in INSPIRE as of 16 Sep 2022

%\cite{Kamionkowski:1993fg}
\bibitem{Kamionkowski:1993fg}
M.~Kamionkowski, A.~Kosowsky and M.~S.~Turner,
%``Gravitational radiation from first order phase transitions,''
Phys. Rev. D \textbf{49}, 2837-2851 (1994)
doi:10.1103/PhysRevD.49.2837
[arXiv:astro-ph/9310044 [astro-ph]].
%605 citations counted in INSPIRE as of 13 Sep 2022

%\cite{Caprini:2019egz}
\bibitem{Caprini:2019egz}
C.~Caprini, M.~Chala, G.~C.~Dorsch, M.~Hindmarsh, S.~J.~Huber, T.~Konstandin, J.~Kozaczuk, G.~Nardini, J.~M.~No and K.~Rummukainen, \textit{et al.}
%``Detecting gravitational waves from cosmological phase transitions with LISA: an update,''
JCAP \textbf{03}, 024 (2020)
doi:10.1088/1475-7516/2020/03/024
[arXiv:1910.13125 [astro-ph.CO]].
%320 citations counted in INSPIRE as of 16 Sep 2022

%\cite{Damour:2000wa}
\bibitem{Damour:2000wa}
T.~Damour and A.~Vilenkin,
%``Gravitational wave bursts from cosmic strings,''
Phys. Rev. Lett. \textbf{85}, 3761-3764 (2000)
doi:10.1103/PhysRevLett.85.3761
[arXiv:gr-qc/0004075 [gr-qc]].
%313 citations counted in INSPIRE as of 05 Sep 2022

%\cite{Damour:2001bk}
\bibitem{Damour:2001bk}
T.~Damour and A.~Vilenkin,
%``Gravitational wave bursts from cusps and kinks on cosmic strings,''
Phys. Rev. D \textbf{64}, 064008 (2001)
doi:10.1103/PhysRevD.64.064008
[arXiv:gr-qc/0104026 [gr-qc]].
%312 citations counted in INSPIRE as of 05 Sep 2022

%\cite{Ringeval:2017eww}
\bibitem{Ringeval:2017eww}
C.~Ringeval and T.~Suyama,
%``Stochastic gravitational waves from cosmic string loops in scaling,''
JCAP \textbf{12}, 027 (2017)
doi:10.1088/1475-7516/2017/12/027
[arXiv:1709.03845 [astro-ph.CO]].
%84 citations counted in INSPIRE as of 05 Sep 2022

%\cite{Cui:2019kkd}
\bibitem{Cui:2019kkd}
Y.~Cui, M.~Lewicki and D.~E.~Morrissey,
%``Gravitational Wave Bursts as Harbingers of Cosmic Strings Diluted by Inflation,''
Phys. Rev. Lett. \textbf{125}, no.21, 211302 (2020)
doi:10.1103/PhysRevLett.125.211302
[arXiv:1912.08832 [hep-ph]].
%31 citations counted in INSPIRE as of 18 Aug 2022
